Are Deep Neural Architectures Losing Information? Invertibility Is Indispensable

Ever since the advent of AlexNet, designing novel deep neural architectures for different tasks has consistently been a productive research direction. Despite the exceptional performance of various architectures in practice, we study a theoretical question: what is the condition for deep neural architectures to preserve all the information of the input data? Identifying the information lossless condition for deep neural architectures is important, because tasks such as image restoration require keep the detailed information of the input data as much as possible. Using the definition of mutual information, we show that: a deep neural architecture can preserve maximum details about the given data if and only if the architecture is invertible. We verify the advantages of our Invertible Restoring Autoencoder (IRAE) network by comparing it with competitive models on three perturbed image restoration tasks: image denoising, jpeg image decompression and image inpainting. Experimental results show that IRAE consistently outperforms non-invertible ones. Our model even contains far fewer parameters. Thus, it may be worthwhile to try replacing standard components of deep neural architectures, such as residual blocks and ReLU, with their invertible counterparts. We believe our work provides a unique perspective and direction for future deep learning research.

==> secs/Architecture.tex <==
\section{Methodology}

\begin{figure}
\centering
\includegraphics[width=\textwidth]{Images/NetArchi2.pdf}
\caption{Glow based Auto-encoder.}
\label{fig:NetArchi}
\vspace{-5mm}
\end{figure}

The contribution of this paper is proposing a new architecture for image restoration.
Our motivation of employing the architecture of Glow is that Glow is invertible, which can encode the complex input distribution to latent variables follow some simple distribution in a lossless way. Thus, we use the invertible layers of Glow as encoder and decoder in our network. However, most image restoration tasks are irreversible. Take image denoising as an example, the same noisy image can correspond to many different clean images given slightly different noise maps. Similarly, the same clean image may correspond to different noisy images with different noise added.
If we only use invertible layers in the network, it can only deal with invertible problems but will be poor at irreversible tasks. Hence, we add irreversible transformation layers between encoder and decoder in our architecture.
As shown in Figure~\ref{fig:NetArchi}, the proposed architecture is composed of three components, encoder, transformation and decoder. This structure is verified applicable to image restoration tasks in our experiment. 

Assume \textbf{y} is the corrupted images and \textbf{x} is the corresponding ground truth. Let $\bm{f_i}$ and $\bm{f_i^'}$ be the invertible transformations in corresponding encoder and decoder layers. The inverse transformation of them are $\bm{f_i}^{-1}$ and $\bm{f_i^'}^{-1}$. We also denote the irreversible functions in the transformation layers as $\bm{t_i}$. 
We use $\bm{h_i}$ and $\bm{h_i}^{-1}$to represent the intermediate variables between the invertible transformations in encoder and decoder. $\bm{z_0}$ is the encoded variable and $\bm{z_i}$ are the intermediate results of the irreversible transformations layers.
The whole process can be described in the flow below.

% \begin{equation*}
% \begin{center}
%     $\bm{y}$ \xleftrightarrow{\text{$\bm{f_1}$}} $\bm{h_1}$ 
%     \xleftrightarrow{\text{$\bm{f_2}$}} $\bm{h_2}$ \dots \xleftrightarrow{\text{$\bm{f_K}$}} $\bm{z_0}$ \xrightarrow{\text{$\bm{t_1}$}} $\bm{z_1}$
%     \xrightarrow{\text{$\bm{t_2}$}} $\bm{z_2}$ \dots 
%     \xrightarrow{\text{$\bm{t_m}$}} $\bm{z_m}$ 
%     \xleftrightarrow{\text{$\bm{f_K^'}^{-1}$}} 
%     % $\bm{h_{K-1}^'}$ 
%     \dots $\bm{h_2^'}$
%     \xleftrightarrow{\text{$\bm{f_2^'}^{-1}$}} $\bm{h_1^'}$ \xleftrightarrow{\text{$\bm{f_1^'}^{-1}$}} $\bm{x}$       
% \end{center}
% \end{equation*}

\subsection{Encoder and Decoder}
The encoder and decoder layers are symmetrical in this architecture, i.e., the number of layers are the same but in a reverse order. 
Both these two modules consist of squeeze layers, step of flow blocks and split layers.

The encoder module maps the corrupted image from a complex and unknown distribution to latent variable $\bm{z_0}$ which follows some distribution in a lower dimension space.
The inverse of the decoder module maps the ground truth image from a different unknown distribution to latent variable $\bm{z_m}$ which follows another distribution in a space with the same dimension as $\bm{z_0}$. Thus, the corrupted image and its corresponding ground truth image are mapped to two different points in a same space. Then, we use the transformation layers to learn the non-linear transformation from a group of points $\bm{z_0}$ (from the corrupted images) to another group of points $\bm{z_m}$ (from the ground truth images) in the same space. If we can learn this mapping successfully, we can restore the ground truth images through decoder. 

\subsection{Transformation}
We employ irreversible layers to learn the non-linear mapping between latent variables $\bm{z_0}$ and $\bm{z_m}$. Since the image restoration tasks are irreversible, these two variables are unlikely to have a one-to-one mapping relationship. These irreversible layers transform $\bm{z_0}$ to the most likely point $\bm{z_m}$ in the same space to restore the given ground truth.

Our transformation module consists of three kinds of layers, i.e., the convolutional layers, Instance Norm layers and Tanh as the activation layers.
% Why use irreversible modules for transformation
\textbf{The convolutional layers} learn affine transformations of the points. 
% Why use InstanceNorm (better than BatchNorm/LayerNorm/GroupNorm)
\textbf{The Instance Norm layers} are used to normalize each point based on the data of that point. Compared with Batch Norm, which normalize each point according to all the data of the corresponding batch, Instance Norm reduces the influence of the bias of the batch while normalizing each point. This will lead to a faster convergence to match the point $\bm{z_0}$ to the corresponding point $\bm{z_m}$.
The selection of \textbf{Tanh} as the activation function is indispensable in this structure, which is important for learning the non-linear mapping between points. Both $\bm{z_0}$ and $\bm{z_m}$ are in the space $[-1,1]^{C\times H\times W}$. Tanh is a zero-centered transformation and can easily map the points in the space of $[-1,1]^{C\times H\times W}$ to other points in the same space, while other activation functions (like Sigmoid and ReLU) will map the points to a different space (like $[0,1]^{C\times H\times W}$), which will severely compromise the learning of mapping.


\subsection{Loss Function}
For image restoration tasks, the relationship of the corrupted image $\textbf{y}$ and the corresponding ground truth image $\textbf{x}$ can be denoted as below.
\begin{equation}
    \bm{y} = A\bm{x}+n
\end{equation}

==> secs/exps_tmp.tex <==
\section{Experiments}
We conduct three experiments to evaluate the image restoration performance of our invertible deep neural architectures: synthetic noise removal, real-image denoising and image inpainting. All these experiments show that our model can consistently restore images to their original forms better than other competitive baseline methods. The quantitative results of synthetic noise removal even show a large-margin improvement. More pleasantly, despite a more superior performance, our invertible architecture contains fewer parameters than other competitive models.

\subsection{Experimental Settings}
For the architecture of InvIR as depicted in Figure x, we apply $K = 16$ and $L = 2$ for the encoding and decoding layers and $B = 5$ for transformation blocks. We adopt Adam as the optimiser. The learning rate is initialised as $10^{-3}$ and decays to $2\times10^{-4}$ after the first 50 epochs. The learning rate decay afterwards is to become a fifth of the original rate if the PSNR does not improve for 10 epochs. We terminate training when the learning rate becomes less than $10^{-6}$.

% Todo: 关于metrics也需要描述一下. 
\subsection{Metrics}
The evaluation metrics we use for comparison are the average peak signal-to-noise ratio (PSNR) and the structural similarity index (SSIM). Higher values indicate better performance for both metrics. 

\begin{table*}[t] %\small
\caption{Quantitative denoising performance of our model compared against others. The column $\sigma$ stands for different noise levels. ``BLD'' represents blind denoising. Values are average PSNR(dB). The best results are highlighted in bold. }
\label{Tab:Synnthetic Denoising}
\centering
\bgroup
\setlength{\tabcolsep}{0.0em}
\begin{tabular}{l@{\quad} |@{\quad} c @{\quad} | @{\quad} c @{\quad} | @{\quad} c @{\quad} |@{\quad} c @{\quad}|@{\quad} c @{\quad}}
\toprule
Dataset & $\sigma$ & DnCNN & FFDNet & Unet & \textbf{Ours} \\ \hline

\multirow{4}{3em}{CelebA} & 15  & 31.4597 & 31.8551 & 31.7719 & 33.0812 \\ 
& 25 & 29.4340 & 28.9438 & 30.5915 & 31.0795 \\ 
& 50 & 26.7126 & 25.5980 & 26.4775 & 28.0887 \\ 
& BLD & 30.3496 & 30.8492 & 30.8807 & 31.6158 \\
\hline
\multirow{4}{3em}{Bird} & 15 & 30.0825 & 31.1383 & 31.9578 & 33.0805 \\
& 25 & 28.4882 & 28.3442 & 30.3652 & 31.0111 \\ 
& 50 & 26.4529 & 26.4082 & 27.7812 & 28.0976 \\ 
& BLD & 28.7662 & 28.4686 & 31.4173 & 31.4448 \\
\hline
\multirow{4}{3em}{Flower} & 15 & 29.8116 & 30.8773 & 32.0690 & 32.6267 \\
& 25 & 28.8444 & 28.2578 & 30.2644 & 30.5044 \\ 
& 50 & 26.1073 & 26.1131 & 27.1729 & 27.5092 \\ 
& BLD & 28.4645 & 28.7165 & 31.3378 & 31.6123 \\
\bottomrule
\end{tabular}
\egroup
\end{table*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{imgs/Denoising.pdf}
    \caption{Qualitative visualisation of image denoising of our model compared with other methods. The noise level $\sigma = 50$. }
    \label{fig:Denoising}
\end{figure}

\subsection{Synthetic Noise Removal}
% Todo: 这个bird数据集是什么样子. 

We first evaluate the denoising capability of our model on three types of images: CelebA (human faces)~\cite{CelebA}, Flower (natural plants)~\cite{Flower} and Bird~\cite{Bird}. The noises are standard additive white Gaussian noises (AWGN), with three distinct standard deviations: $\sigma=15, 25, 50$. We also conduct experiments for blind denoising with random noise levels between 0 to 55. \autoref{Tab:Synnthetic Denoising} quantitatively demonstrate that our model perform denoising better than other approaches with a large margin. \autoref{fig:Denoising} exhibits qualitative results of the denoising performance of our model compared against others. 

\textbf{Comparisons of parameters and convergence speed.}
We use a 40 layer DnCNN. The comparison of number of parameters is listed in Table~\ref{Tab:Face Denoising Performance Comparision}. Our structure achieves higher denoising accuracy with less parameters compared with DnCNN and Unet.

% \begin{table*}[t]
% \caption{Peformance Comparison on CelebA.}
% \label{Tab:Face Denoising Performance Comparision}
% \centering
% \begin{tabular}{l|c|c|c|c}
% \hline\hline
% Methods & DnCNN & Unet & GAE (w/o T) & GAE (T) \\ \hline
% % & GAE (with Trans) \\ \hline
% Number of Parameters & $1.48\times10^6$ & $7.70\times10^6$ & $1.33\times10^6$ & $1.33\times10^6$ \\ 
% Inference Time & 0.25 & 0.44 & 0.59 & 1.83\\
% \hline\hline
% \end{tabular}
% \end{table*}

\begin{table*}[t] %\small
\caption{Peformance Comparison on CelebA.}
\label{Tab:Face Denoising Performance Comparision}
\centering
\bgroup
\setlength{\tabcolsep}{0.0em}
\begin{tabular}{l@{\quad} |@{\quad} c @{\quad} | @{\quad} c @{\quad}| @{\quad} c @{\quad}}
\toprule
Dataset & DnCNN & Unet & \textbf{Ours} \\ \hline
Number of Parameters & $1.48\times10^6$ & $7.70\times10^6$ & $1.33\times10^6$ \\ 
Inference Time & 0.25 & 0.44 & 1.83\\
\bottomrule
\end{tabular}
\egroup
\end{table*}

\begin{figure}
\begin{centering}
\includegraphics[width=0.8\textwidth]{Images/Denoise_Convergence.pdf}
\caption{Convergence Speed Comparison.}
\label{fig:Convergence}
\end{centering}
\end{figure}

\begin{comment}
\subsection{Real Noise Removing}
We also conduct real noise removing on the real noise dataset SIDD. During training, we randomly crop $80\times80$ patches from each images in the training set.
% DnD~\cite{Tobias_2017_CVPR} and SIDD~\cite{SIDD_2018_CVPR}.
% Following the method of generating training set in the work RIDNet~\cite{RIDNet}, CBDNet~\cite{Guo2019Cbdnet} and FFDNet~\cite{zhang2018ffdnet}, we randomly cropped 2000 $512\times512$ patch pairs
% The training set is randomly cropped from three real noise datasets, \ie SIDD~\cite{SIDD_2018_CVPR}, PolyU~\cite{PolyU} and Renoir~\cite{anaya2014renoir}, resulting in 2000 $512\times512$ patch pairs for training. This strategy of generating training set follows RIDNet~\cite{RIDNet}, CBDNet~\cite{Guo2019Cbdnet} and FFDNet~\cite{zhang2018ffdnet}, which not only increase the diversity of noise and texture distributions exposed to the network but also keep the training size not too large to save the training time. 
% These patches are randomly cropped into $80\times80$ patches during training. 

\textbf{Quantitative results.}
The comparison of our architecture with the state-of-arts are listed in Table~\ref{Tab:SIDD}

\textbf{Qualitative results.}
\end{comment}

\textbf{Comparisons of parameters and convergence speed.}

% \begin{table*}[t]\small       
% \caption{Real image denoising on SIDD.}
% \label{Tab:SIDD}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \hline\hline
% Methods & BM3D~\cite{BM3D} & CBDNet~\cite{Guo2019Cbdnet} & AINDNet~\cite{AINDNet} & VDN~\cite{VDN} & CycleISP~\cite{CycleISP} & GAE (w/o T) & GAE (T) \\ \hline
% PSNR & 25.65 & 33.28 & 39.08 & 39.26 & 39.52 & 38.7 & 39.20 \\ \hline
% SSIM & 0.685 & 0.868 & 0.953 & 0.955 & 0.957 & & \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

\begin{table*}[t] %\small
\caption{Real image denoising on SIDD.}
\label{Tab:Face Denoising Performance Comparision}
\centering
\bgroup
\setlength{\tabcolsep}{0.0em}
\begin{tabular}{l@{\quad} |@{\quad} c @{\quad} | @{\quad} c @{\quad}| @{\quad} c @{\quad}|@{\quad} c @{\quad} | @{\quad} c @{\quad}| @{\quad} c @{\quad}| @{\quad} c @{\quad}}
\toprule
Methods & BM3D~\cite{BM3D} & CBDNet~\cite{Guo2019Cbdnet} & AINDNet~\cite{AINDNet} & VDN~\cite{VDN} & CycleISP~\cite{CycleISP} & GAE (w/o T) & GAE (T) \\ \hline
PSNR & 25.65 & 33.28 & 39.08 & 39.26 & 39.52 & 38.7 & 39.20 \\ \hline
SSIM & 0.685 & 0.868 & 0.953 & 0.955 & 0.957 & & \\
\bottomrule
\end{tabular}
\egroup
\end{table*}

% \begin{table*}\small      
% \caption{Real image denoising on DND.}
% \label{Tab:Blind Denoising}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \hline\hline
% Methods & CIMM~\cite{CIMM} & RIDNet~\cite{RIDNet} & AINDNet~\cite{AINDNet} & VDN~\cite{VDN} & CycleISP~\cite{CycleISP} & GAE (w/o T) & GAE (T) \\ \hline
% PSNR & 39.20 & 39.26 & 39.7695 & 39.383 & 39.56 & &  \\ \hline
% SSIM & 0.9524 & 0.9528 & 0.959 & 0.9518 & 0.9564 & & \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

% \begin{table*}[t] %\small
% \centering
% % \resizebox{\columnwidth}{!}{
% \begin{tabular}{l|c|c|c|c}
% \hline\hline
% \multirow{2}{2em}{Method} & \multicolumn{2}{c|}{DnD} & \multicolumn{2}{c}{SIDD}\\
% \cline{2-5}
%  & PSNR & SSIM & PSNR & SSIM \\
% \hline\hline
% DnCNN~\cite{DnCNN} &  32.43 & 0.7900 & 23.66 & 0.583 \\ \hline
% %EPLL & Non-Blind & 33.51 & 0.8244 & 27.11 & 0.870 \\ \hline
% TNRD~\cite{TNRD} & 33.65 & 0.8306 & 24.73 & 0.643 \\ \hline
% %NCSR & Non-Blind & 34.05 & 0.8351 \\ \hline
% %MLP &  & 34.23 & 0.8331 & 24.71 & 0.641 \\ \hline
% FFDNet~\cite{zhang2018ffdnet} & 34.40 & 0.8474 & -- & -- \\ \hline
% BM3D~\cite{BM3D} & 34.51 & 0.8507 & 25.65 & 0.685 \\ \hline
% %FoE & Non-Blind & 34.62 & 0.8845 \\ \hline
% %WNNM & Non-Blind & 34.67 & 0.8646 & 25.78 & 0.809 \\ \hline
% %DenoiseNet & \textcolor{red}{Blind} & 35.08 & 0.868 \\ \hline
% NI & 35.11 & 0.8778 & -- & -- \\ \hline
% NC~\cite{NC} & 35.43 & 0.8841 & -- & -- \\ \hline
% %GCBD & \checkmark & 35.58 & 0.9217 \\ \hline
% KSVD~\cite{KSVD} & 36.49 & 0.8978 & 26.88 & 0.842 \\ \hline
% %KSVD-G & -- & -- & 27.19 & 0.771 \\ \hline
% %KSVD-DCT & -- & -- & 27.51 & 0.780 \\ \hline
% %MCWNNM & & 37.38 & 0.9294 \\ \hline
% %FFDNet+ & Non-Blind & 37.61 & 0.9415 \\ \hline
% %DnCNN+ & \checkmark & 37.90 & 0.943 \\ \hline
% TWSC~\cite{TWSC} & 37.96 & 0.9416 & -- & -- \\ \hline
% CBDNet~\cite{Guo2019Cbdnet} & 38.06 & 0.9421 & 33.28 & 0.868 \\ \hline
% %PD & \checkmark & 38.40 & 0.9452 \\ \hline
% %NLH & \checkmark & 38.81 & 0.952 \\ \hline
% %WDnCNN+ & \checkmark & 38.87  & 0.9501  \\ \hline
% %ATDNet & \checkmark & 39.19 & 0.9526  \\ \hline
% CIMM~\cite{CIMM} & 39.20  & 0.9524 & -- & -- \\ \hline
% MLDN & 39.23  & 0.9516 & -- & -- \\ \hline
% RIDNet~\cite{RIDNet} & 39.26 & 0.9528 & -- & -- \\ \hline
% % VDN & \checkmark & 39.38 & 0.9518 \\ \hline
% PRIDNet~\cite{PRID_net} & 39.42 & 0.9528 & -- & -- \\ \hline
% DRDN~\cite{DRDN} & 39.43 & 0.9531 & -- & -- \\ \hline
% % DeepProxies BM3D &--&--& 34.34 & 0.911 \\ \hline
% Path-Restore~\cite{yu2019pathrestore} & 39.7227 & 0.9591 & 38.21 & 0.946 \\ \hline
% % DNW-Baseline & 39.1503 & 0.9521 & 38.30 & 0.948  \\ \hline
% % BoostNet & -- & -- & 38.57 & 0.950 \\ \hline
% KPCN~\cite{KPCN} & -- & -- & 38.60 & 0.948 \\ \hline
% % HI-GAN~\cite{} & 39.3683 & 0.9542 & 38.88 & 0.952 \\ \hline
% % UNet_D & -- & -- & 38.88 & 0.952 \\ \hline
% % URDNet_boostnet & -- & -- & 38.88 & 0.952 \\ \hline
% AINDNet~\cite{AINDNet} & 39.7695 & 0.959 & 39.08 & 0.953 \\ \hline
% VDN~\cite{VDN} & 39.383 & 0.9518 & 39.26 & 0.955 \\ \hline
% CycleISP~\cite{CycleISP} & 39.5649 & 0.9564 & 39.52 & 0.957 \\ \hline
% % MIRNet~\cite{} & 39.88 & 0.9563 & -- & -- \\ \hline
% % HT-MWResnet~\cite{} & 39.8447& 0.958 & 39.80 & 0.959 \\ \hline
% GAE (w/o Trans) & & & & \\ \hline
% GAE (with Trans) &  &  & 38.47 &  \\ \hline \hline
% \end{tabular}
% % }
% % \vspace{-2mm}
% \caption{Method comparison on the DnD sRGB and SIDD sRGB datasets. The mean PSNR and SSIM are reported.}%denoising results of algorithms evaluated on the DnD sRGB and SIDD sRGB datasets}
% \label{Tab:DnD_SIDD}
% \vspace{-1em}
% \end{table*}


% The PSNR comparisons are in Table 3. C-Glow producesreasonably good results. However, it is worse than DnCNNand BM3D. To further analyze c-Glow’s performance, weshow  qualitative  results  in  Figure  3.  One  main  reason  thePSNR of c-Glow is lower than DnCNN is that the imagesgenerated  by  DnCNN  are  smoother  than  the  images  gen-erated by c-Glow. We believe this is caused by one draw-back of flow-based models. Flow-based models use squeeze layers to fold input tensors to exploit the local correlation structure of an image. The squeeze layers use a spatial pixel-wise checkerboard mask to split the input tensor, which may cause values of neighbor pixels to vary non-smoothly.

\subsection{Image Inpainting}
% Inferring parts of images that are censored or occluded re-quires modeling of the structure of dependencies across pix-els. In this set of experiments, we test c-Glow on the taskof inpainting censored images from the CelebA dataset (Liuet al. 2015), which has around 200,000 images of faces. Werandomly select 2,000 images as our test set. We centrallycrop the images and resize them to64×64pixels. We usecentral block masks such that25\%of the pixels are hiddenfrom the input. For c-Glow, we setL= 3,K= 8,nc= 64,andnw= 128.  For  training  the  model,  we  set  the  fea-turesxto  be  the  occluded  images  and  the  labelsyto  bethe  center  region  that  needs  to  be  inpainted.  We  compareour method with DCGAN inpainting (DCGANi) (Yeh et al 2017),  which  is  the  state-of-the-art  deep  model  for  imageinpainting. We use PSNR as our metric.

% \begin{table*}[t]
% \caption{Image inpainting on CelebA.}
% \label{Tab:CBSD68,Kodak24,McM}
% \centering
% \begin{tabular}{l|c|c|c|c|c}
% \hline\hline
% Method & DCGANi & DCGANi-b & c-Glow & Unet & GAE \\ \hline
% PSNR & 22.73 & 23.65 & 24.88 & 36.91 & 34.96 \\
% \hline\hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

% \begin{table*}[t]\small
% \caption{Image impainting on CelebA with centering holes. CA is . SH is . PC is Partial Conv~\cite{}. GC is Gated Conv~\cite{}. CSA is Coherent Semantic Attention~\cite{}.SF is structure Flow~\cite{}.The numbers are from CSA paper.}
% \label{Tab:Center_holes}
% \centering
% \begin{tabular}{l|c|c|c|c|c}
% \hline\hline
% % Dataset & \multicolumn{4}{c|}{CelebA}&
% % \multicolumn{4}{c}{Flower} \\ \hline
% \multirow{2}{5em}{Method} & Contextual Attention & Shift-net & Coherent Semantic & GAE (w/o T) & GAE (T\_I)   \\
% & ~\cite{} & ~\cite{} & Attention~\cite{} & &   \\\hline
% PSNR & 23.93 & 26.38 & 26.54 & 27.14 &  \\ \hline
% SSIM & 0.882 & 0.926 & 0.931 & 0.975 & \\ \hline
% % L1 Loss (\%) & & 2.64 & 1.97 & 1.83 & & \\ \hline
% % L2 Loss (\%) & & 0.47 & 0.28 & 0.27 & & \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

\begin{table*}[t] %\small
\caption{Image impainting on CelebA with centering holes. CA is . SH is . PC is Partial Conv~\cite{}. GC is Gated Conv~\cite{}. CSA is Coherent Semantic Attention~\cite{}.SF is structure Flow~\cite{}.The numbers are from CSA paper.}
\label{Tab:Center_holes}
\centering
\bgroup
\setlength{\tabcolsep}{0.0em}
\begin{tabular}{l@{\quad} |@{\quad} c @{\quad} | @{\quad} c @{\quad}| @{\quad} c @{\quad}|@{\quad} c @{\quad}}
\toprule
\multirow{2}{5em}{Method} & Contextual Attention & Shift-net & Coherent Semantic & \textbf{Ours}  \\
& ~\cite{} & ~\cite{} & Attention~\cite{}&  \\\hline
PSNR & 23.93 & 26.38 & 26.54 & 27.14  \\ \hline
SSIM & 0.882 & 0.926 & 0.931 & 0.975 \\
\bottomrule
\end{tabular}
\egroup
\end{table*}

% \begin{table*}[t]\small
% \caption{Image impainting on CelebA with irregular holes.}
% \label{Tab:irreguar_holes}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c}
% \hline\hline
% % Dataset & \multicolumn{4}{c|}{CelebA}&
% % \multicolumn{4}{c}{Flower} \\ \hline
% Method & Mask & PC & GC & CSA & GAE (w/o T) & GAE (T\_I)  \\ \hline
% \multirow{3}{5em}{PSNR} & 10-20\% & 31.13 & 31.67 & 34.69 & 36.33 &  \\
% & 20-30\% & 29.10 & 29.83 & 32.58 & 32.57 &  \\
% & 30-40\% & 23.46 & 24.48 & 25.32 & 27.53 &  \\ 
% & 40-50\% & 22.11 & 23.36 & 24.14 & 24.18 &  \\ \hline
% \multirow{3}{5em}{SSIM} & 10-20\% & 0.970 & 0.977 & 0.989 & 0.993 &  \\
% & 20-30\% & 0.956 & 0.964 & 0.982 & 0.984 &  \\
% & 30-40\% & 0.897 & 0.910 & 0.926 & 0.955 &  \\ 
% & 40-50\% & 0.839 & 0.860 & 0.883 & 0.926 &  \\ \hline
% % \multirow{3}{5em}{L1 Loss (\%)} & 10-20\% & 1.00 & 1.00 & & 0.72 & &  \\
% % & 20-30\% & 1.46 & 1.40 & & 0.94 & &  \\
% % & 30-40\% & 2.97 & 2.62 & & 2.18 & &  \\ 
% % & 40-50\% & 4.01 & 3.26 & & 2.85 & &  \\ \hline
% % \multirow{3}{5em}{L2 Loss (\%)} & 10-20\% & 0.12 & 0.08 & & 0.04 & &  \\
% % & 20-30\% & 0.19 & 0.12 & & 0.07 & &  \\
% % & 30-40\% & 0.58 & 0.44 & & 0.37 & &  \\ 
% % & 40-50\% & 0.76 & 0.50 & & 0.44 & &  \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

\begin{table*}[t] %\small
\caption{Image impainting on CelebA with irregular holes.}
\label{Tab:irreguar_holes}
\centering
\bgroup
\setlength{\tabcolsep}{0.0em}
\begin{tabular}{l@{\quad} |@{\quad} c @{\quad} | @{\quad} c @{\quad}| @{\quad} c @{\quad}|@{\quad} c @{\quad}| @{\quad} c @{\quad}}
\toprule
Method & Mask & PC & GC & CSA & \textbf{Ours}\\ \hline
\multirow{3}{5em}{PSNR} & 10-20\% & 31.13 & 31.67 & 34.69 & 36.33\\
& 20-30\% & 29.10 & 29.83 & 32.58 & 32.57  \\
& 30-40\% & 23.46 & 24.48 & 25.32 & 27.53  \\ 
& 40-50\% & 22.11 & 23.36 & 24.14 & 24.18  \\ \hline
\multirow{3}{5em}{SSIM} & 10-20\% & 0.970 & 0.977 & 0.989 & 0.993  \\
& 20-30\% & 0.956 & 0.964 & 0.982 & 0.984 \\
& 30-40\% & 0.897 & 0.910 & 0.926 & 0.955 \\ 
& 40-50\% & 0.839 & 0.860 & 0.883 & 0.926 \\
\bottomrule
\end{tabular}
\egroup
\end{table*}

The network is also evaluated on image inpainting task. We employ the CelebA dataset and use the original train, validation and test splits in our training. Experiments on both settings of center and irregular holes are conducted. All the images for training and testing are reshaped to the size of $256\times 256$. These images are randomly cropped into $64\times64$ patches during training. For the setting of center hole, we generate $128 \times 128$ rectangular masks on a random position which is close to the center of images for the training and test set. For the setting of irregular hole, the irregular masks are obtained from the work of Partial Conv~\cite{}. 

Our model is optimized by Adam with the default hyperparameters and a learning rate $1\times 10^{-4}$. We train two architectures, GAE with $K=8$ and $L=3$ for the encoder and decoder layers (GAE(w/o T)) and the same GAE with $B=5$ for transformation blocks (GAE(T\_I)). 

We also conduct real noise removing on two real noise datasets, DnD~\cite{Tobias_2017_CVPR} and SIDD~\cite{SIDD_2018_CVPR}. 
The training set is randomly cropped from three real noise datasets, \ie SIDD~\cite{SIDD_2018_CVPR}, PolyU~\cite{PolyU} and Renoir~\cite{anaya2014renoir}, resulting in 2000 $512\times512$ patch pairs for training. This strategy of generating training set follows RIDNet~\cite{RIDNet}, CBDNet~\cite{Guo2019Cbdnet} and FFDNet~\cite{zhang2018ffdnet}, which not only increase the diversity of noise and texture distributions exposed to the network but also keep the training size not too large to save the training time. 

\textbf{Quantitative results.}
We randomly select 500 images from Celeba validation
dataset [27] and generate irregular and centering holes for
each image to make comparisons. Following the CA [42],
we use common evaluation metrics, i.e., L1, L2, PSNR, and
SSIM to quantify the performance of the models. Table 1
and Table 2 list the evaluation results with centering mask
and irregular masks respectively. It can be seen that our
method outperforms all the other methods on these measurements with irregular mask or centering mask.
Based on the hole-to-image area ratios, these masks are classified to different groups, such as 10\%-20\%. Following the work of CSA~\cite{}, we report the results on 4 of these groups, i.e., 10\%-20\%, 20\%-30\%, 30\%-40\% and 40\%-50\%.
The comparison of our architecture with the state-of-arts are listed in Table~\ref{Tab:Center_holes}

\textbf{Qualitative results.}

% \begin{table*}[t]\small                                               
% \caption{Image impainting on Places2 with centering holes. CA is Contextual Attention~\cite{}. SH is Shift-net~\cite{}. PC is Partial Conv~\cite{}. GC is Gated Conv~\cite{}. CSA is Coherent Semantic Attention~\cite{}.}
% \label{Tab:Synnthetic Denoising}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c}
% \hline\hline
% % Dataset & \multicolumn{4}{c|}{CelebA}&
% % \multicolumn{4}{c}{Flower} \\ \hline
% Method & CA~\cite{} & SH~\cite{} & PC~\cite{} & GC~\cite{} & CSA~\cite{} & GAE (w/o T) & GAE (T\_I) & GAE (T\_II)   \\ \hline
% PSNR &  &  & &  &  & &  & \\ \hline
% SSIM &  &  & &  &  & & & \\ \hline
% L1 Loss (\%) &  &  &  &  &  &  & \\ \hline
% L2 Loss (\%) & &  &  &  &  &  & \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

% \begin{table*}[t]\small                                               
% \caption{Image impainting on irregular holes.}
% \label{Tab:Synnthetic Denoising}
% \centering
% \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c}
% \hline\hline
% % Dataset & \multicolumn{4}{c|}{CelebA}&
% % \multicolumn{4}{c}{Flower} \\ \hline
% Dataset & Mask & CA & SH & PC & GC & P-Unet & CSA & StructureFlow & GAE (w/o T) & GAE (T\_I) & GAE (T\_II)   \\ \hline
% \multirow{3}{5em}{CelebA} & 10-20\% & & & 31.13 & 31.67 & & 34.69 & & &  & \\
% & 20-30\% &  &  & 29.10 & 29.83 & & 32.58 & & &  & \\
% & 30-40\% &  & & 23.46 & 24.48 & & 25.32 & & &  & \\ 
% & 40-50\% &  & & 22.11 & 23.36 & & 24.14 & & &  & \\ \hline
% \multirow{3}{5em}{Place2} & 10-20\% & 26.27 & & 31.030 & & &  & 32.029 & &  & \\
% & 20-30\% & 24.21 &  & 23.673 & &&  & 25.218 & &  & \\
% & 30-40\% & 21.95 &  & 23.673 & &&  & 25.218 & &  & \\
% & 40-50\% & 20.02 & & 19.743 & &&  & 21.090 & &  & \\ \hline
% % \multirow{3}{5em}{Paris Street View} & 10-20\% &  & & & &  & & & &  & \\
% % & 20-30\% &  &  & &  & & & & & & \\
% % & 30-40\% &  & & &  & & & &  &  & \\ 
% % & 40-50\% &  & & &  & & & &  & & \\ \hline
% \hline
% \end{tabular}
% % \vspace{-2mm}
% % \vspace{-1.2em}
% \end{table*}

% % Todo: 把这个表格描述清楚. 
% \begin{table}[t]
% \caption{JPEG Image Deblocking.}
% \label{Tab:JPEG_Deblocking}
% \centering
% \begin{tabular}{l|c|c|c|c}
% \hline\hline
% % \multicolumn{1}{l|}{\multirow{2}{*}{Dataset}}&
% \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Quality \\ Metrics\end{tabular}}} & \multicolumn{1}{c|}{AR-CNN} & \multicolumn{1}{c|}{DnCNN} & \multicolumn{1}{c|}{Unet}  &\multicolumn{1}{c}{\textbf{InvIR (Ours)}}  \\ 

% & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c|}{PSNR/SSIM} & \multicolumn{1}{c}{PSNR/SSIM} \\ \hline

% 10 & 27.8221/0.9368 & 27.5406/0.9326 & 28.7041/0.9479 & \textbf{28.7322/0.9476} \\ 
% % & 
% 20 & 29.9814/0.9568 & 28.8870/0.9469 & 30.9274/0.9647 & \textbf{30.9984/0.9652} \\
% % & 
% 30 & 31.1935/0.9658 & 28.6428/0.9350 & 32.0025/0.9712 & \textbf{32.1832/0.9715} \\
% % & 
% 40 & 31.9283/0.9702 & 31.0741/0.9648 & 32.8755/0.9757 & \textbf{33.0835/0.9765} \\ \hline
% \hline
% \end{tabular}
% \end{table}

\begin{table*}[t] %\small
\caption{Image impainting on CelebA with irregular holes.}
\label{Tab:irreguar_holes}
\centering
\bgroup
\setlength{\tabcolsep}{0.0em}
\begin{tabular}{l@{\quad} |@{\quad} c @{\quad} | @{\quad} c @{\quad}| @{\quad} c @{\quad}|@{\quad} c @{\quad}}
\toprule
{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Quality \\ Metrics\end{tabular}}} & 
AR-CNN & DnCNN & UNet & \textbf{Ours} \\
& PSNR/SSIM & PSNR/SSIM & PSNR/SSIM & PSNR/SSIM \\ \hline 
10 & 27.8221/0.9368 & 27.5406/0.9326 & 28.7041/0.9479 & \textbf{28.7322/0.9476} \\ 
20 & 29.9814/0.9568 & 28.8870/0.9469 & 30.9274/0.9647 & \textbf{30.9984/0.9652} \\
30 & 31.1935/0.9658 & 28.6428/0.9350 & 32.0025/0.9712 & \textbf{32.1832/0.9715} \\
40 & 31.9283/0.9702 & 31.0741/0.9648 & 32.8755/0.9757 & \textbf{33.0835/0.9765} \\
\bottomrule
\end{tabular}
\egroup
\end{table*}

\subsection{JPEG Image Decompression}
We evaluate the capability of our model on decompressing JPEG images. JPEG is a commonly used lossy image compression method. It achieves compression by converting images into the frequency domain, followed by discarding the high-frequency regions that are hard to perceive by humans. However, JPEG compression often leads to artefacts, such as block noise and mosquito noise. Our model can reconstruct JPEG images back to their original forms. The effectiveness can be supported by 



==> secs/intro.tex <==
\section{Introduction}
Ever since AlexNet won the ImageNet challenge in 2012 \cite{krizhevsky2012imagenet}, deep learning has been revolutionizing research in many industries~\cite{lecun2015deep}. One important reason for the success of deep learning is due to the transferability of the architectures \cite{vaswani2017attention} \ie a model architecture that is suitable for one task can also perform well for a variety of other related tasks. For example, the convolutional neural networks (CNNs) designed for image classification also demonstrate pleasing performance acting as a generator for generative adversarial networks (GANs) \cite{radford2015unsupervised}. Similarly, recurrent neural networks (RNNs) that are commonly applied for modeling languages or other sequences \cite{levy2014neural} have recently also been employed to generate graphs \cite{you2018graphrnn}.

% Thanks to AlexNet winning the ImageNet challenge in 2012 \cite{krizhevsky2012imagenet}, deep learning has been revolutionising almost all industries \cite{lecun2015deep}. One vital reason for the success of deep learning dues to the transferability of its architectures \cite{vaswani2017attention}. That is, a model architecture that is suitable for one task can also perform well for a variety of other related tasks. For example, the convolutional neural networks (CNN) designed for image classification also demonstrate pleasing performance acting as a generator for generative adversarial networks (GAN) \cite{radford2015unsupervised}. Furthermore, recurrent neural networks (RNN) are commonly applied for modelling languages or other sequences \cite{levy2014neural}. Recently, they are also employed to generate graphs \cite{you2018graphrnn}.

The majority of deep learning architectures were initially proposed to address high-level computer vision tasks \cite{szegedy2015going}, \eg CNNs originally emerged as a method for recognizing hand-written characters \cite{lecun2015lenet}. Recently, following the success of AlexNet for image classification, different deep architectures have been invented for various high-level vision tasks, such as Region-CNN (R-CNN) for detection \cite{girshick2014rich} and residual network (ResNet) \cite{he2016deep} for classification. Inspired by the great achievements of deep architectures in high-level vision tasks, researchers also explored applying these deep architectures in low-level vision tasks and achieved satisfactory performance. For example, SRCNN \cite{dong2015image} and DnCNN \cite{zhang2017beyond} achieved superior accuracy in image super-resolution and denoising respectively, in comparison to traditional methods.

% The majority of deep learning architectures are initially proposed to address high-level computer vision tasks \cite{szegedy2015going}. For example, CNNs originally emerge for recognising hand-written digits \cite{lecun2015lenet}. Recently, following the success of AlexNet for image classification as mentioned above, different deep architectures have been invented for various high-level vision tasks, such as Region-CNN (R-CNN) for detection \cite{girshick2014rich} and residual networks (ResNet) \cite{he2016deep} for even better classification performance. Inspired by the great achievements of deep architectures in high-level vision tasks, researchers also explore applying these deep architectures in low-level vision tasks and also receive satisfying performance. For example, SRCNN \cite{dong2015image} and DnCNN \cite{zhang2017beyond} achieve superior accuracy in image super-resolution and denoising separately.
% 超分和降噪都有什么工作. 

Nonetheless, there is a division between the requirements for deep models for high- and low-level vision tasks. It may be acceptable to miss image details for high-level tasks, as long as it captures the most salient features. However, missing details of images can be unsupportable when dealing with low-level vision tasks \cite{zhang2020residual}. Instead of primarily concentrating on conceptual vision features, the latter systems require specific minutiae such as colors and textures to be able to restore original images \cite{liu2020gradnet}. 

% Nonetheless, there is a division between the requirements for deep models of high and low-level vision tasks. It might be acceptable to miss image details for high-level tasks, so long as the most salient features are captured by the system. However, this detail missing of images can be intolerable when dealing with low-level tasks \cite{zhang2020residual}. The latter systems, instead of mainly concentrating on conceptual vision features, demand primarily specific minutiae such as colours and textures in order to restore the original images \cite{liu2020gradnet}. 

Inspired by this division, we study the appropriateness of applying deep architectures of high-level vision tasks to tackle low-level tasks. We show theoretically that common architectures such as ResNet and components such as ReLU can lead to information loss about the input images. Therefore, they are not desirable for tasks which require the preservation of input details. Fortunately, we derive characteristics of deep architectures that are theoretically guaranteed for no information loss, what we call lossless deep architectures. In summary, our contributions are three-fold: 
\vspace{-2.05mm}
\begin{enumerate}
    \item From the perspective of information theory, we show non-invertible deep architectures lead to loss of information concerning the input. 
    \item Inspired by the need for invertibility, we develop an Invertible Restoring Autoencoder (IRAE) network via invertible flow-based generative algorithms.  
    \item We test IRAE with a series of experiments, finding that we achieve superior performance on both image denoising and inpainting tasks. Moreover, our models have fewer parameters than the baseline lossy models. 
\end{enumerate}
% Inspired by such a division, in this paper, we study the appropriateness of applying deep architectures of high-level vision tasks to tackle low-level ones. We show in theory that common architectures such as ResNet and ReLU can lead to information loss about the input images. Therefore, they are not desirable for preserving input details. Fortunately, we derive characteristics of deep architectures that are theoretically guaranteed for no information loss. In summary, our contributions are three-folds: 
% \begin{enumerate}
%     \item From the perspective of information theory, we show non-invertible deep architectures lead to losing information about the input. 
%     \item Inspired by the necessity of invertibility, we build image-restoration models based on flow-based generative models since the latter ones also require invertible deep architectures, following exactly the same spirit with our theoretical demand.  
%     \item We test our model on a battery of experiments. We achieve better performance on both image denoising and inpainting tasks. More pleasingly, our model has fewer parameters than baselines. 
% \end{enumerate}

\begin{comment}
Except for AlexNet for image classification mentioned above, CNN originally adverts for recognising hand-written digits. Furthermore, Region-CNN (R-CNN) and 

In this paper, we study 

We prove that skip-connection structures such as residual blocks can cause the loss of information as the data flows in a deep neural network.

We devise an architecture 

Experiments 


Image denoising has consistently been a vital problem since the inception of computer vision and image processing~\cite{chang2000adaptive,xu2017multi}. Nearly all traditional industries demand reliable image denoising techniques for conducting safe and efficient activities. Immediate examples include denoising medical images to assist doctors diagnosing deceases more accurately and enhancing the quality of photos of crime suspects to support better social justice. Some future technologies are also highly dependant on image denoising techniques. For example, poor image denoising performance at night can cause inferior recognition of pedestrians for autonomous vehicles. This recognition defect can lead to catastrophic human injuries.

Traditional image denoising techniques are closely related to signal processing approaches, such as learned simultaneous sparse coding and cascade of shrinkage fields. Despite these methods have achieved reasonably good denoising performance, they suffer from non-generalisability and non-end-to-end. Specifically, a certain model can only tackle a particular denoising task. Furthermore, a model requires a lot of manual setting in order to achieve desirable performance. 

In the past decade, starting from AlexNet winning the ImageNet challenge in 2012, deep learning has revolutionised a lot of research fields. Consequently, researchers start applying deep learning models in image denoising. 

Despite great successes, the

The majority of CNN architectures are designed to address high-level tasks such as image classification and object detection. Such high-level tasks do not pay a lot of attention on image details such as textures and colours. However, these details play an essential role in image denoising. 

Therefore, image denoising requires deep architectures that can preserve detailed information. Inspired by this requirement, we resort to deep generative models. These models aim to produce images that look similar to the original given data. Thus, they are required to maintain as much information as possible to reconstruct the realistic images. 

Flow-based generative models are gaining more and more popularity. 

Such models are conceptually attractive since there exists an exact mapping between the input data and the latent representations. As such, there is no information loss for encoding an image to its latent vector as well as for the reverse process. Such an architecture is a perfect candidate acting as a deep image denoising model.

Flow-based generative models share the same spirit as image denoising models.

We summarise our contributions as follows: 
1. 
2. 
3. 
\end{comment}
